Local Linear Convergence of Approximate Projections onto Regularized Sets

The numerical properties of algorithms for finding the intersection of sets depend to some extent on the regularity of the sets, but even more importantly on the regularity of the intersection. The alternating projection algorithm of von Neumann has been shown to converge locally at a linear rate dependent on the regularity modulus of the intersection. In many applications, however, the sets in question come from inexact measurements that are matched to idealized models. It is unlikely that any such problems in applications will enjoy metrically regular intersection, let alone set intersection. We explore a regularization strategy that generates an intersection with the desired regularity properties. The regularization, however, can lead to a significant increase in computational complexity. In a further refinement, we investigate and prove linear convergence of an approximate alternating projection algorithm. The analysis provides a regularization strategy that fits naturally with many ill-posed inverse problems, and a mathematically sound stopping criterion for extrapolated, approximate algorithms. The theory is demonstrated on the phase retrieval problem with experimental data. The conventional early termination applied in practice to unregularized, consistent problems in diffraction imaging can be justified fully in the framework of this analysis providing, for the first time, proof of convergence of alternating approximate projections for finite dimensional, consistent phase retrieval problems.

==> drlmacros.tex <==
%--------------------------
% page settings
%--------------------------
% \topmargin 0.0cm
% \oddsidemargin -0.1cm
% \textwidth  16.4cm 
% \headheight 0.0cm
% \textheight 21.7cm
% \parindent  6mm
% \parskip    10pt
% \tolerance  1000

%--------------------------
%  PACKAGES
%--------------------------
%

% SIAM compatible packages:
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage[pdftex]{graphicx}
\usepackage{graphicx}
% \usepackage{exscale,cmmib57}
\usepackage{exscale,relsize}
\usepackage{amsfonts}
% \usepackage{fontenc}

% SIAM doesn't like the following:
% \usepackage{calc}
\usepackage{cite}
% \usepackage{changebar}
\usepackage{theorem} %
% \usepackage{amsthm}
% \usepackage{pifont}      %needed by dingautolist
% \usepackage{fancybox}
% \usepackage{latexsym}

% Autographia packages
% \usepackage[latin1]{inputenc}
% \usepackage[francais]{babel}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Generates hyperlinked PDF:
\RequirePackage{hyperref}
\PassOptionsToPackage{pdftex,bookmarksopen,bookmarksnumbered}{hyperref}
\voffset=-0.5in
  %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{hyperref}

% INDEXING COMMANDS
\usepackage{makeidx}
\newcommand{\idxdef}[1]{\textbf{\hyperpage{#1}}}
\newcommand{\idxquo}[1]{\hyperpage{#1}$\dag$}
\newcommand{\idxfig}[1]{\hyperpage{#1}$\ddag$}


%--------------------------
%  MACROS
%--------------------------
%
% Theorems
%
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{propn}[thm]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
\newtheorem{defn}[thm]{Definition}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{condition}[thm]{Condition}
\newtheorem{conjecture}[thm]{Conjecture}
\theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{alg}[thm]{Algorithm}
\theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{algorithm}[thm]{Algorithm}
\theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{eg}[thm]{Example}
\theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\newtheorem{remark}[thm]{Remark}
% \theoremstyle{plain}{\theorembodyfont{\rmfamily}%
\def\proof{\noindent{\it Proof}. \ignorespaces}
\def\endproof{\vbox{\hrule height0.6pt\hbox{\vrule height1.3ex%
width0.6pt\hskip0.8ex\vrule width0.6pt}\hrule height0.6pt}\medskip}
\renewcommand{\labelenumi}{\rm (\arabic{enumi})}
\renewcommand{\labelenumii}{\rm (\alph{enumii})}
\numberwithin{equation}{section}
% reference:
\newcommand{\eqr}[1]{Eq.(\ref{#1})}
\newcommand{\figr}[1]{Figure \ref{#1}}

% %Detailed calculations not meant for publication:
% \newcommand{\detail}[1]{\par\noi{\bf [Proof detail\ }{#1}
% \hfill{\bf ]}\par\noi\hspace{-4pt}}
% \renewcommand{\detail}[1]{}
% 
% 
% use as
% 
% \detail{ text }
% 
% lines:
% \rule[4pt]{6.8in}{0.05cm}\\


%-------------------------------
% Fonts and accents
%-------------------------------
%
% caligraphic:
\newcommand{\Acal}{{\mathcal A}}
\newcommand{\Bcal}{{\mathcal B}}
\newcommand{\Ccal}{{\mathcal C}}
\newcommand{\Dcal}{{\mathcal D}}
\newcommand{\Ecal}{{\mathcal E}}
\newcommand{\Fcal}{{\mathcal F}}
\newcommand{\Gcal}{{\mathcal G}}
\newcommand{\Hcal}{{\mathcal H}}
\newcommand{\Ical}{{\mathcal I}}
\newcommand{\Jcal}{{\mathcal J}}
\newcommand{\Kcal}{{\mathcal K}}
\newcommand{\Lcal}{{\mathcal L}}
\newcommand{\Mcal}{{\mathcal M}}
\newcommand{\Ncal}{{\mathcal N}}
\newcommand{\Ocal}{{\mathcal O}}
\newcommand{\Pcal}{{\mathcal P}}
\newcommand{\Qcal}{{\mathcal Q}}
\newcommand{\Rcal}{{\mathcal R}}
\newcommand{\Scal}{{\mathcal S}}
\newcommand{\Tcal}{{\mathcal T}}
\newcommand{\Ucal}{{\mathcal U}}
\newcommand{\Vcal}{{\mathcal V}}
\newcommand{\Wcal}{{\mathcal W}}
\newcommand{\Ycal}{{\mathcal Y}}
\newcommand{\Xcal}{{\mathcal X}}
\newcommand{\Zcal}{{\mathcal Z}}
\newcommand{\acal}{{\mathcal a}}

% mathbb
\newcommand{\Abb}{\mathbb{A}}
\renewcommand{\Bbb}{\mathbb{B}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Dbb}{\mathbb{D}}
\newcommand{\Ebb}{\mathbb{E}}
\newcommand{\Fbb}{\mathbb{F}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Ibb}{\mathbb{I}}
\newcommand{\Jbb}{\mathbb{J}}
\newcommand{\Kbb}{\mathbb{K}}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Obb}{\mathbb{O}}
\newcommand{\Pbb}{\mathbb{P}}
\newcommand{\Qbb}{\mathbb{Q}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Tbb}{\mathbb{T}}
\newcommand{\Ubb}{\mathbb{U}}
\newcommand{\Vbb}{\mathbb{V}}
\newcommand{\Wbb}{\mathbb{W}}
\newcommand{\Xbb}{\mathbb{X}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Zbb}{\mathbb{Z}}

% hats
\newcommand{\Ahat}{{\widehat{A}}}
\newcommand{\Bhat}{{\widehat{B}}}
\newcommand{\Chat}{{\widehat{C}}}
\newcommand{\Dhat}{{\widehat{D}}}
\newcommand{\Ehat}{{\widehat{E}}}
\newcommand{\Fhat}{{\widehat{F}}}
\newcommand{\Ghat}{{\widehat{G}}}
\newcommand{\Hhat}{{\widehat{H}}}
\newcommand{\Ihat}{{\widehat{I}}}
\newcommand{\Jhat}{{\widehat{J}}}
\newcommand{\Khat}{{\widehat{K}}}
\newcommand{\Lhat}{{\widehat{L}}}
\newcommand{\Mhat}{{\widehat{M}}}
\newcommand{\Nhat}{{\widehat{N}}}
\newcommand{\Phat}{{\widehat{P}}}
\newcommand{\Qhat}{{\widehat{Q}}}
\newcommand{\Rhat}{{\widehat{R}}}
\newcommand{\Shat}{{\widehat{S}}}
\newcommand{\That}{{\widehat{T}}}
\newcommand{\Uhat}{{\widehat{U}}}
\newcommand{\Vhat}{{\widehat{V}}}
\newcommand{\What}{{\widehat{W}}}
\newcommand{\Xhat}{{\widehat{X}}}
\newcommand{\Yhat}{{\widehat{Y}}}
\newcommand{\Zhat}{{\widehat{Z}}}
\newcommand{\ahat}{{\widehat{a}}}
\newcommand{\bhat}{{\widehat{b}}}
\newcommand{\chat}{{\widehat{c}}}
\newcommand{\dhat}{{\widehat{d}}}
\newcommand{\ehat}{{\widehat{e}}}
\newcommand{\fhat}{{\widehat{f}}}
\newcommand{\ghat}{{\widehat{g}}}
\newcommand{\hhat}{{\widehat{h}}}
\newcommand{\ihat}{{\widehat{i}}}
\newcommand{\jhat}{{\widehat{j}}}
\newcommand{\khat}{{\widehat{k}}}
\newcommand{\lhat}{{\widehat{l}}}
\newcommand{\mhat}{{\widehat{m}}}
\newcommand{\nhat}{{\widehat{n}}}
\newcommand{\phat}{{\widehat{p}}}
\newcommand{\qhat}{{\widehat{q}}}
\newcommand{\rhat}{{\widehat{r}}}
\newcommand{\shat}{{\widehat{s}}}
\newcommand{\that}{{\widehat{t}}}
\newcommand{\uhat}{{\widehat{u}}}
\newcommand{\vhat}{{\widehat{v}}}
\newcommand{\what}{{\widehat{w}}}
\newcommand{\xhat}{{\widehat{x}}}
\newcommand{\yhat}{{\widehat{y}}}
\newcommand{\zhat}{{\widehat{z}}}

\newcommand{\alphahat}{{\widehat{\alpha}}}
\newcommand{\betahat}{{\widehat{\beta}}}
\newcommand{\gammahat}{{\widehat{\gamma}}}
\newcommand{\deltahat}{{\widehat{\delta}}}
\newcommand{\etahat}{{\widehat{\eta}}}
\newcommand{\kappahat}{{\widehat{\kappa}}}
\newcommand{\phihat}{{\widehat{\phi}}}
\newcommand{\psihat}{{\widehat{\psi}}}
\newcommand{\sigmahat}{{\widehat{\sigma}}}
\newcommand{\Omegahat}{{\widehat{\Omega}}}
\newcommand{\omegahat}{{\widehat{\omega}}}

% bars
\newcommand{\Abar}{{\overline{A}}}
\newcommand{\Bbar}{{\overline{B}}}
\newcommand{\Cbar}{{\overline{C}}}
\newcommand{\Dbar}{{\overline{D}}}
\newcommand{\Ebar}{{\overline{E}}}
\newcommand{\Fbar}{{\overline{F}}}
\newcommand{\Gbar}{{\overline{G}}}
\newcommand{\Hbar}{{\overline{H}}}
\newcommand{\Ibar}{{\overline{I}}}
\newcommand{\Jbar}{{\overline{J}}}
\newcommand{\Kbar}{{\overline{K}}}
\newcommand{\Lbar}{{\overline{L}}}
\newcommand{\Mbar}{{\overline{M}}}
\newcommand{\Nbar}{{\overline{N}}}
\newcommand{\Pbar}{{\overline{P}}}
\newcommand{\Qbar}{{\overline{Q}}}
\newcommand{\Rbar}{{\overline{R}}}
\newcommand{\Sbar}{{\overline{S}}}
\newcommand{\Tbar}{{\overline{T}}}
\newcommand{\Ubar}{{\overline{U}}}
\newcommand{\Vbar}{{\overline{V}}}
\newcommand{\Wbar}{{\overline{W}}}
\newcommand{\Xbar}{{\overline{X}}}
\newcommand{\Ybar}{{\overline{Y}}}
\newcommand{\Zbar}{{\overline{Z}}}
\newcommand{\abar}{{\overline{a}}}
\newcommand{\bbar}{{\overline{b}}}
\newcommand{\cbar}{{\overline{c}}}
\newcommand{\dbar}{{\overline{d}}}
\newcommand{\ebar}{{\overline{e}}}
\newcommand{\fbar}{{\overline{f}}}
\newcommand{\gbar}{{\overline{g}}}
% \newcommand{\hbar}{{\overline{h}}}
\newcommand{\ibar}{{\overline{i}}}
\newcommand{\jbar}{{\overline{j}}}
\newcommand{\kbar}{{\overline{k}}}
\newcommand{\lbar}{{\overline{l}}}
\newcommand{\mbar}{{\overline{m}}}
\newcommand{\nbar}{{\overline{n}}}
\newcommand{\pbar}{{\overline{p}}}
\newcommand{\qbar}{{\overline{q}}}
\newcommand{\rbar}{{\overline{r}}}
\newcommand{\sbar}{{\overline{s}}}
\newcommand{\tbar}{{\overline{t}}}
\newcommand{\ubar}{{\overline{u}}}
\newcommand{\vbar}{{\overline{v}}}
\newcommand{\wbar}{{\overline{w}}}
\newcommand{\xbar}{{\overline{x}}}
\newcommand{\ybar}{{\overline{y}}}
\newcommand{\zbar}{{\overline{z}}}

\newcommand{\alphabar}{{\overline{\alpha}}}
\newcommand{\betabar}{{\overline{\beta}}}
\newcommand{\nubar}{{\overline{\nu}}}
\newcommand{\mubar}{{\overline{\mu}}}
\newcommand{\gammabar}{{\overline{\gamma}}}
\newcommand{\epsilonbar}{{\overline{\epsilon}}}
\newcommand{\deltabar}{{\overline{\delta}}}
\newcommand{\etabar}{{\overline{\eta}}}
\newcommand{\kappabar}{{\overline{\kappa}}}
\newcommand{\lambdabar}{{\overline{\lambda}}}
\newcommand{\phibar}{{\overline{\phi}}}
\newcommand{\psibar}{{\overline{\psi}}}
\newcommand{\thetabar}{{\overline{\theta}}}
\newcommand{\zetabar}{{\overline{\zeta}}}
\newcommand{\Omegabar}{{\overline{\Omega}}}

% tildes
\newcommand{\Atilde}{{\widetilde{A}}}
\newcommand{\Btilde}{{\widetilde{B}}}
\newcommand{\Ctilde}{{\widetilde{C}}}
\newcommand{\Dtilde}{{\widetilde{D}}}
\newcommand{\Etilde}{{\widetilde{E}}}
\newcommand{\Ftilde}{{\widetilde{F}}}
\newcommand{\Gtilde}{{\widetilde{G}}}
\newcommand{\Htilde}{{\widetilde{H}}}
\newcommand{\Itilde}{{\widetilde{I}}}
\newcommand{\Jtilde}{{\widetilde{J}}}
\newcommand{\Ktilde}{{\widetilde{K}}}
\newcommand{\Ltilde}{{\widetilde{L}}}
\newcommand{\Mtilde}{{\widetilde{M}}}
\newcommand{\Ntilde}{{\widetilde{N}}}
\newcommand{\Ptilde}{{\widetilde{P}}}
\newcommand{\Qtilde}{{\widetilde{Q}}}
\newcommand{\Rtilde}{{\widetilde{R}}}
\newcommand{\Stilde}{{\widetilde{S}}}
\newcommand{\Ttilde}{{\widetilde{T}}}
\newcommand{\Utilde}{{\widetilde{U}}}
\newcommand{\Vtilde}{{\widetilde{V}}}
\newcommand{\Wtilde}{{\widetilde{W}}}
\newcommand{\Xtilde}{{\widetilde{X}}}
\newcommand{\Ytilde}{{\widetilde{Y}}}
\newcommand{\Ztilde}{{\widetilde{Z}}}
\newcommand{\atilde}{{\widetilde{a}}}
\newcommand{\btilde}{{\widetilde{b}}}
\newcommand{\ctilde}{{\widetilde{c}}}
\newcommand{\dtilde}{{\widetilde{d}}}
\newcommand{\etilde}{{\widetilde{e}}}
\newcommand{\ftilde}{{\widetilde{f}}}
\newcommand{\gtilde}{{\widetilde{g}}}
\newcommand{\htilde}{{\widetilde{h}}}
\newcommand{\itilde}{{\widetilde{i}}}
\newcommand{\jtilde}{{\widetilde{j}}}
\newcommand{\ktilde}{{\widetilde{k}}}
\newcommand{\ltilde}{{\widetilde{l}}}
\newcommand{\mtilde}{{\widetilde{m}}}
\newcommand{\ntilde}{{\widetilde{n}}}
\newcommand{\ptilde}{{\widetilde{p}}}
\newcommand{\qtilde}{{\widetilde{q}}}
\newcommand{\rtilde}{{\widetilde{r}}}
\newcommand{\stilde}{{\widetilde{s}}}
\newcommand{\ttilde}{{\widetilde{t}}}
\newcommand{\utilde}{{\widetilde{u}}}
\newcommand{\vtilde}{{\widetilde{v}}}
\newcommand{\wtilde}{{\widetilde{w}}}
\newcommand{\xtilde}{{\widetilde{x}}}
\newcommand{\ytilde}{{\widetilde{y}}}
\newcommand{\ztilde}{{\widetilde{z}}}

\newcommand{\alphatilde}{{\widetilde{\alpha}}}
\newcommand{\betatilde}{{\widetilde{\beta}}}
\newcommand{\gammatilde}{{\widetilde{\gamma}}}
\newcommand{\deltatilde}{{\widetilde{\delta}}}
\newcommand{\etatilde}{{\widetilde{\eta}}}
\newcommand{\kappatilde}{{\widetilde{\kappa}}}
\newcommand{\phitilde}{{\widetilde{\phi}}}
\newcommand{\psitilde}{{\widetilde{\psi}}}
\newcommand{\zetatilde}{{\widetilde{\zeta}}}
\newcommand{\Omegatilde}{{\widetilde{\Omega}}}
\newcommand{\Psitilde}{{\widetilde{\Psi}}}
\newcommand{\Phitilde}{{\widetilde{\Phi}}}

% boldface
\newcommand{\Abf}{{\bf{A}}}
\newcommand{\Bbf}{{\bf{B}}}
\newcommand{\Cbf}{{\bf{C}}}
\newcommand{\Dbf}{{\bf{D}}}
\newcommand{\Ebf}{{\bf{E}}}
\newcommand{\Fbf}{{\bf{F}}}
\newcommand{\Gbf}{{\bf{G}}}
\newcommand{\Hbf}{{\bf{H}}}
\newcommand{\Ibf}{{\bf{I}}}
\newcommand{\Jbf}{{\bf{J}}}
\newcommand{\Kbf}{{\bf{K}}}
\newcommand{\Lbf}{{\bf{L}}}
\newcommand{\Mbf}{{\bf{M}}}
\newcommand{\Nbf}{{\bf{N}}}
\newcommand{\Pbf}{{\bf{P}}}
\newcommand{\Qbf}{{\bf{Q}}}
\newcommand{\Rbf}{{\bf{R}}}
\newcommand{\Sbf}{{\bf{S}}}
\newcommand{\Tbf}{{\bf{T}}}
\newcommand{\Ubf}{{\bf{U}}}
\newcommand{\Vbf}{{\bf{V}}}
\newcommand{\Wbf}{{\bf{W}}}
\newcommand{\Xbf}{{\bf{X}}}
\newcommand{\Ybf}{{\bf{Y}}}
\newcommand{\Zbf}{{\bf{Z}}}
\newcommand{\abf}{{\bf{a}}}
\newcommand{\bbf}{{\bf{b}}}
\newcommand{\cbf}{{\bf{c}}}
\newcommand{\dbf}{{\bf{d}}}
\newcommand{\ebf}{{\bf{e}}}
\newcommand{\fbf}{{\bf{f}}}
\newcommand{\gbf}{{\bf{g}}}
% \newcommand{\hbf}{{\bf{h}}}
\newcommand{\ibf}{{\bf{i}}}
\newcommand{\jbf}{{\bf{j}}}
\newcommand{\kbf}{{\bf{k}}}
\newcommand{\lbf}{{\bf{l}}}
\newcommand{\mbf}{{\bf{m}}}
\newcommand{\nbf}{{\bf{n}}}
\newcommand{\pbf}{{\bf{p}}}
\newcommand{\qbf}{{\bf{q}}}
\newcommand{\rbf}{{\bf{r}}}
\newcommand{\sbf}{{\bf{s}}}
\newcommand{\tbf}{{\bf{t}}}
\newcommand{\ubf}{{\bf{u}}}
\newcommand{\vbf}{{\bf{v}}}
\newcommand{\wbf}{{\bf{w}}}
\newcommand{\xbf}{{\bf{x}}}
\newcommand{\ybf}{{\bf{y}}}
\newcommand{\zbf}{{\bf{z}}}

\newcommand{\alphabf}{{\bf{\alpha}}}
\newcommand{\betabf}{{\bf{\beta}}}
\newcommand{\nubf}{{\bf{\nu}}}
\newcommand{\gammabf}{{\bf{\gamma}}}
\newcommand{\deltabf}{{\bf{\delta}}}
\newcommand{\etabf}{{\bf{\eta}}}
\newcommand{\kappabf}{{\bf{\kappa}}}
\newcommand{\lambdabf}{{\bf{\lambda}}}
\newcommand{\phibf}{{\bf{\phi}}}
\newcommand{\psibf}{{\bf{\psi}}}
\newcommand{\zetabf}{{\bf{\zeta}}}
\newcommand{\Omegabf}{{\bf{\Omega}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% oft used constructs and miscellany:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% General:
\def\Upon#1#2{ {{\displaystyle #1}\over {\displaystyle #2}} }
\renewcommand{\Im}{{\rm Im}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\equiv}{:=}
\newcommand{\cint}{\circ\!\!\!\!\!\int}
\newcommand{\toinf}{\rightarrow\infty}
\newcommand{\tozero}{\rightarrow 0}
\newcommand{\attains}[1]{\rightarrow_{\!\!\!\!\!\!\!{_#1}}~}
\newcommand{\emp}{\ensuremath{\text{{\sffamily\O}}}}
\newcommand{\Ball}{{\Bbb}}
\newcommand{\ball}{{\Bbb}}
\newcommand{\Rn}{{\Rbb^n}}
\newcommand{\Rnp}{{\Rbb^n_+}}
\newcommand{\Rnn}{{\Rbb^{n\times n}}}
\newcommand{\Rmn}{{\Rbb^{m\times n}}}
\newcommand{\Rm}{{\Rbb^m}}
\newcommand{\Rk}{{\Rbb^k}}
\newcommand{\Rp}{{\Rbb_+}}
\newcommand{\Rth}{{\Rbb^3}}
\newcommand{\Rtw}{{\Rbb^2}}
\newcommand{\extre}{(-\infty,+\infty]}
\newcommand{\extrem}{[-\infty,+\infty]}
\newcommand{\cc}[1]{\overline{#1}}
\newcommand{\ucmin}[2]{\underset{#2}{\mbox{minimize}}~#1}
\newcommand{\argucmin}[2]{\underset{#2}{\mbox{argmin}}~#1}
\newcommand{\cmin}[3]{\begin{array}{ll}\underset{#2}{\mbox{minimize }}\qquad #1&\\
                       \mbox{subject to }\qquad#3&\end{array}}

\newcommand{\ucmax}[2]{\underset{#2}{\mbox{maximize}}~#1}
\newcommand{\cmax}[3]{\begin{array}{ll}\underset{#2}{\mbox{maximize }}\qquad #1&\\
                       \mbox{subject to }\qquad#3&\end{array}}
\newcommand{\set}[2]{\left\{#1\,\left|\,#2\right.\right\}}
\newcommand{\map}[3]{#1:\,#2\rightarrow #3\,}
\newcommand{\mmap}[3]{#1:\,#2\rightrightarrows #3\,}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pdn}[2]{\frac{\partial^n #1}{\partial #2^n}}
\newcommand{\D}[2]{\frac{d #1}{d #2}}
\newcommand{\DD}[2]{\frac{d^2 #1}{d #2^2}}
\newcommand{\Dn}[2]{\frac{d^n #1}{d #2^n}}

\newcommand{\vect}[1]{{\boldsymbol #1}}
\newcommand{\ip}[2]{\left\langle #1,~ #2\right\rangle}
\newcommand{\twxo}[2]{\left(\begin{array}{c}#1 \\#2\end{array}\right)}
\newcommand{\thxo}[3]{\left(\begin{array}{c}#1 \\#2\end{array}\right)}
\newcommand{\thxth}[9]{\left(\begin{array}{ccc}#1 &#2&#3\\#4 &#5&#6\\#7 &#8&#9\end{array}\right)}
\newcommand{\twxtw}[4]{\left(\begin{array}{cc}#1 &#2\\#3&#4\end{array}\right)}
\newcommand{\normsq}[1]{\left\|#1\right\|^2}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norminf}[1]{\left\|#1\right\|_{\infty}}
\newcommand{\itr}[2]{{#1_{{#2}}}}
\newcommand{\seq}[1]{{(\itr{#1}{n})_{n\in\Nbb}}}
\newcommand{\range}[1]{{\rm range}(#1)}

\newcommand{\comp}[1]{#1^{\circ}}
\renewcommand{\choose}[2]{\left(\begin{array}{c}\!#1\!\\\!#2\!\end{array}\right)}
\newcommand{\modu}{\!\!\!\!\!\mod\!}
\newcommand{\as}{\qquad\mbox{a.s.}}
\newcommand{\asto}{\overset{a.s.}{\to}}
\newcommand{\im}{{\rm {\scriptstyle i}}}
\newcommand{\und}{\quad\mbox{ and }\quad}
\newcommand{\where}{\quad\mbox{ where }\quad}
\newcommand{\fur}{\mbox{ for }}
\newcommand{\ow}{\mbox{ otherwise }}
\newcommand{\bdy}{\partial}
\newcommand{\spcl}[1]{{{#1}_*}}
% \newcommand{\qed}{\hfill $\Box$ \\ \medskip}

% Variational Analysis:
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\limi}{\varliminf}
\DeclareMathOperator{\lims}{\varlimsup}
\DeclareMathOperator{\weakly}{\rightharpoonup}
\DeclareMathOperator{\weakstarly}{\stackrel{\mathrm{w*}}{\rightharpoondown}}
\DeclareMathOperator{\xtoinf}{\|\text{$x$}\| \rightarrow +\infty}
\DeclareMathOperator{\sgn}{sign\,}
\DeclareMathOperator{\sinc}{sinc\,}
\DeclareMathOperator{\argmax}{argmax\,}
\DeclareMathOperator{\argmin}{argmin\,}
\DeclareMathOperator{\dist}{dist \;}
\DeclareMathOperator{\kernel}{null\,}
\DeclareMathOperator{\dir}{dir\,}
\DeclareMathOperator{\lev}{{lev\,}}
\DeclareMathOperator{\cone}{{cone\,}}
\DeclareMathOperator{\dom}{{dom\,}}
\DeclareMathOperator{\gph}{gph}
% \DeclareMathOperator{\supp}{supp\,} % siam doesn't like this
\DeclareMathOperator{\conv}{conv\,}
\DeclareMathOperator{\hull}{co\,}
\DeclareMathOperator{\intr}{int\,}
\DeclareMathOperator{\cont}{cont\,}
\DeclareMathOperator{\core}{core\,}
\DeclareMathOperator{\trace}{{\bf Tr}\,}
\DeclareMathOperator{\diag}{Diag\,} % siam doesn't like this
\DeclareMathOperator{\Fix}{\mathsf{Fix}\,}
\newcommand{\epi}[1]{{\mbox{epi}\, #1}}
\newcommand{\sepi}[1]{{\mbox{\scriptsize epi}\, (#1)}}
\newcommand{\tcone}[2]{{T}_{#2}(#1)}
\newcommand{\ncone}[2]{{N}_{#2}(#1)}
\newcommand{\rncone}[2]{\widehat{{N}}_{#2}(#1)}
\newcommand{\cl}{\mbox{\rm cl}\,}
\newcommand{\wstcl}[1]{{\mbox{{\rm cl}}^*\left( #1\right)}}
\newcommand{\wcl}{{\mbox{cl}^*\,}}
\newcommand{\closu}[1]{\ensuremath{\overline{#1}}}
% \newcommand{\intr}[1]{{\mbox{int}\;#1}}
\newcommand{\ri}[1]{{\mbox{ri}\;#1}}
\newcommand{\polar}[1]{{\left( #1\right)^\circ}}
\newcommand{\support}[1]{{\psi^*_{#1}}}
\newcommand{\sd}{\partial}
\newcommand{\csd}{{\overline\partial}}
\newcommand{\rsd}{{\widehat\partial}}
\newcommand{\rsg}{{\widehat d}}

% Scattering:
\newcommand{\uinf}{u^{\infty}}
\newcommand{\us}{u^{s}}
\newcommand{\ui}{u^{i}}
\newcommand{\winf}{w^{\infty}}
\newcommand{\ws}{w^{s}}
\newcommand{\wi}{w^{i}}
\newcommand{\vinf}{v^{\infty}}
\newcommand{\vs}{v^{s}}
\newcommand{\vi}{v^{i}}
\newcommand{\ps}{\Phi}             % point source
\newcommand{\psinf}{\Phi{^\infty}}  % far field pattern of point source
\newcommand{\di}{\etahat}              % incident field direction
\newcommand{\scd}{\Omega}                           % scattering domain (assumed closed)
\newcommand{\oexter}{\scd^o}   % open exterior of scattering domain
\newcommand{\exter}{\cl{\scd^o}}   % open exterior of scattering domain
\newcommand{\bdyint}[1]{\int_{\!\bdy #1}}

%
%=========================================
%    End macros
%=========================================


